Practical Computation of Graph VC-Dimension

For any set system $H=(V,R), \ R \subseteq 2^V$, a subset $S \subseteq V$ is called \emph{shattered} if every $S' \subseteq S$ results from the intersection of $S$ with some set in $\R$. The \emph{VC-dimension} of $H$ is the size of a largest shattered set in $V$. In this paper, we focus on the problem of computing the VC-dimension of graphs. In particular, given a graph $G=(V,E)$, the VC-dimension of $G$ is defined as the VC-dimension of $(V, \mathcal N)$, where $\mathcal N$ contains each subset of $V$ that can be obtained as the closed neighborhood of some vertex $v \in V$ in $G$. Our main contribution is an algorithm for computing the VC-dimension of any graph, whose effectiveness is shown through experiments on various types of practical graphs, including graphs with millions of vertices. A key aspect of its efficiency resides in the fact that practical graphs have small VC-dimension, up to 8 in our experiments. As a side-product, we present several new bounds relating the graph VC-dimension to other classical graph theoretical notions. We also establish the $W[1]$-hardness of the graph VC-dimension problem by extending a previous result for arbitrary set systems.

==> tbls/bounds-loc.tex <==
\hline
\textbf{graph} & \textbf{lb64} & \textbf{loc-lb} & \textbf{VCdim} & \textbf{loc-ub} & \textbf{deg-ub} & \textbf{n-ub} & \textbf{degen+1} & \textbf{time}\\
\hline
BIO-MV-Physical-3.5 & 5 & 5 & \textbf{5} & 9 & 11 & 14 & 37 & 0.23\\
BIO-SYS-Aff-Cap-MS-3.5 & 7 & 6 & \textbf{7} & 12 & 12 & 15 & 52 & 1.20\\
BIO-SYS-Aff-Cap-RNA-3.5 & 6 & 7 & \textbf{7} & 10 & 12 & 13 & 55 & 0.41\\
dip20170205 & 5 & 5 & \textbf{5} & 8 & 9 & 14 & 22 & 0.30\\
\hline
oregon2-010331 & 5 & 5 & \textbf{6} & 10 & 12 & 13 & 32 & 0.10\\
CAIDA-as-20130601 & 6 & 6 & \textbf{7} & 12 & 12 & 15 & 69 & 1.25\\
DIMES-201204 & 7 & 6 & \textbf{7} & 12 & 12 & 14 & 35 & 0.54\\
as-skitter & 8 & 8 & \textbf{8} & 16 & 16 & 20 & 112 & 1072.02\\
\hline
p2p-Gnutella09 & 5 & 5 & \textbf{5} & 7 & 7 & 12 & 11 & 0.04\\
gnutella31 & 3 & 4 & \textbf{4} & 6 & 7 & 15 & 7 & 1.27\\
notreDame & 4 & 4 & \textbf{6} & 13 & 14 & 18 & 156 & 37.01\\
y-BerkStan & 7 & 5 & \textbf{7} & 14 & 17 & 19 & 202 & 327.45\\
\hline
ca-HepPh & 5 & 4 & \textbf{5} & 9 & 9 & 13 & 239 & 0.25\\
com-dblp & 4 & 4 & \textbf{5} & 9 & 9 & 18 & 114 & 32.41\\
epinions1 & 7 & 7 & \textbf{7} & 12 & 12 & 16 & 68 & 2.88\\
facebook-combined & 6 & 4 & \textbf{6} & 9 & 11 & 11 & 116 & 0.16\\
twitter-combined & 6 & 7 & \textbf{7} & 12 & 12 & 16 & 97 & 5.25\\
\hline
t.CAL & 3 & 3 & \textbf{3} & 3 & 4 & 20 & 4 & 1110.98\\
t.FLA & 3 & 3 & \textbf{3} & 3 & 4 & 20 & 4 & 357.65\\
buddha & 3 & 4 & \textbf{4} & 4 & 5 & 19 & 6 & 95.00\\
froz & 3 & 2 & \textbf{3} & 4 & 4 & 19 & 5 & 178.46\\
z-alue7065 & 3 & 3 & \textbf{3} & 3 & 3 & 15 & 3 & 0.38\\
\hline
grid300-10 & 3 & 3 & \textbf{3} & 3 & 3 & 16 & 3 & 2.58\\
xgrid500-10 & 3 & 3 & \textbf{3} & 3 & 3 & 17 & 3 & 18.95\\
powerlaw2.5 & 6 & 6 & \textbf{6} & 14 & 14 & 19 & 19 & 325.77\\
\hline

